Learning to Generate Image Embeddings with User-level Differential Privacy

Small on-device models have been successfully trained with user-level differential privacy (DP) for next word prediction and image classification tasks in the past. However, existing methods can fail when directly applied to learn embedding models using supervised training data with a large class space. To achieve user-level DP for large image-to-embedding feature extractors, we propose DP-FedEmb, a variant of federated learning algorithms with per-user sensitivity control and noise addition, to train from user-partitioned data centralized in the datacenter. DP-FedEmb combines virtual clients, partial aggregation, private local fine-tuning, and public pretraining to achieve strong privacy utility trade-offs. We apply DP-FedEmb to train image embedding models for faces, landmarks and natural species, and demonstrate its superior utility under same privacy budget on benchmark datasets DigiFace, EMNIST, GLD and iNaturalist. We further illustrate it is possible to achieve strong user-level DP guarantees of $\epsilon<4$ while controlling the utility drop within 5%, when millions of users can participate in training.

==> exp_param_freeze_app.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htb]
\centering
\begin{subfigure}[b]{0.21\textwidth}
\centering
\includegraphics[width=\textwidth]{figs2/digi-freeze-util.pdf}
\caption{}
\label{fig:digi-freeze-util}
\end{subfigure}
% 
\begin{subfigure}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figs2/digi-freeze-noise.pdf}
\caption{}
\label{fig:digi-freeze-noise}
\end{subfigure}
%
\begin{subfigure}[b]{0.25\textwidth}
\centering
\includegraphics[width=\textwidth]{figs2/digi-mobilenet-noise.pdf}
\caption{}
\label{fig:digi-mobilenet-noise2}
\end{subfigure}
%
\begin{subfigure}[b]{0.21\textwidth}
\centering
\includegraphics[width=\textwidth]{figs2/digi-abl-pretr.pdf}
\caption{}
\label{fig:digi-abl-pretr2}
\end{subfigure}
\caption{ \Ourmetric on DigiFace validation set when training (a) a ResNet with partial frozen parameters for $800$ rounds without noise;
(b) a partially frozen ResNet with \ouralg; (c) a MobileNet with \ouralg w/ pretraining, and baselines of DP-\fedavg and \ouralg w/o pretraining; (d) a MobileNet with different pretrained models. 
}
\label{fig:digi-freeze2}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%

\input{exp_param_freeze_text}

==> exp_roc_curves_app.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htb]
\centering
\begin{subfigure}[b]{0.31\textwidth}
\centering
\includegraphics[width=\textwidth]{figs2/digi-training-curve.pdf}
\caption{}
\label{fig:digi-training-curve_2}
\end{subfigure}
% 
\begin{subfigure}[b]{0.32\textwidth}
\centering
\includegraphics[width=\textwidth]{figs2/test-roc-small-noise.pdf}
\caption{}
\label{fig:digi-sn-roc}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\textwidth}
\centering
\includegraphics[width=\textwidth]{figs2/test-roc-median-noise.pdf}
\caption{}
\label{fig:digi-ln-roc_2}
\end{subfigure}
\caption{ \ouralg and DP-\fedavg on DigiFace10K under the same privacy budget, and additional oracle baseline of centralized training w/o DP: (a) \ourmetric on validation dataset during training, and dashed lines are approximation by sampling a subset of validation users; (b) and (c) ROC curve of trained model on test set, with noise multiplier $0.02$ and $0.08$, respectively; the x-axis in (b) and (c) are in logarithmic scale.
}
\label{fig:curve-roc2_2}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%

==> exp_table_add_app.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htb]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{Dataset} & \multirow{2}{*}{Algorithm} & \multicolumn{4}{c|}{Hyperparameters} & \multicolumn{2}{c|}{Recall@FAR=$1\mathrm{e}{-3}$ / $0.1$}  \\ 
    \cline{3-8} 
    & & Noise & \text{SerLR} & \text{CliLR}  & \text{Clip} & Approx  & AllPair  \\ 
    \hline
    \multirow{2}{*}{DigiFace} & DP-FedEmb &  \multirow{2}{*}{$1.39$} & $5\mathrm{e}{-3}$ &\multirow{2}{*}{$2\mathrm{e}{-3}$} & $0.5$ & - & $19.76\pm0.43$  \\
     & DP-FedAvg &  & $2\mathrm{e}{-3}$ & & $1.5$ & - &  $13.38\pm0.27$ \\
    \hline
    \multirow{2}{*}{EMNIST} & DP-FedEmb & \multirow{2}{*}{$0.62$} & \multirow{2}{*}{$0.02$} & \multirow{2}{*}{$5\mathrm{e}{-3}$} & \multirow{2}{*}{$1$} & $10.64\pm0.5$ & $10.47\pm0.5$\\
     & DP-FedAvg & & & & & $9.78\pm0.44$ & $9.67\pm0.41$ \\
    \hline
    \multirow{2}{*}{GLD} & DP-FedEmb &  \multirow{2}{*}{$0.02$} & 1 &\multirow{2}{*}{$5\mathrm{e}{-4}$} & $0.3$ & $26.18\pm0.44$ & $27.07\pm0.04$ \\
     & DP-FedAvg &  & $0.5$ & & $0.7$ & $24.48\pm1.0$ &  $26.27\pm0.17$ \\
    \hline
    \multirow{2}{*}{iNat} & DP-FedEmb & \multirow{2}{*}{$0.5$} & $0.02$ & $5\mathrm{e}{-4}$  & $0.2$ &  $40.49\pm1.08$  & $40.93\pm0.94$  \\
     & DP-FedAvg &  & $0.01$ & $1\mathrm{e}{-3}$ & $1$  & $29.57\pm0.78$  & $29.6\pm0.65$ \\
    \hline
    \end{tabular}
    \caption{The utility under same privacy budget for DigiFace \citep{bae2023digiface1m}, EMNIST \citep{emnist}, GLD \citep{gldv2}, and iNat \citep{inat} datasets.} 
    \label{tab:additional2_2}
\end{table*}
%%%%%%%%%%%%%%%%

For EMNIST, we train the embedding model on images of class $0-35$ and test on images of class $36-62$. Using a relatively large noise multiplier $0.62$ for $200$ rounds, and sampling $8$ users per virtual client and $32$ virtual clients per round, $\epsilon=9.28,\delta=10^{-4}$ can be achieved given $6800$ users. A small nework with two convolutional layers similar to LeNet \citep{lecun1998gradient} is used as the backbone network, and no pretrained model is used for initialization. We provide results on EMNIST primarily for reproducibility as the scale of EMNIST is smaller than the other datasets used in this draft. 
